Fundamental Limits for Sensor-Based Robot Control

Our goal is to develop theory and algorithms for establishing fundamental limits on performance imposed by a robot's sensors for a given task. In order to achieve this, we define a quantity that captures the amount of task-relevant information provided by a sensor. Using a novel version of the generalized Fano inequality from information theory, we demonstrate that this quantity provides an upper bound on the highest achievable expected reward for one-step decision making tasks. We then extend this bound to multi-step problems via a dynamic programming approach. We present algorithms for numerically computing the resulting bounds, and demonstrate our approach on three examples: (i) the lava problem from the literature on partially observable Markov decision processes, (ii) an example with continuous state and observation spaces corresponding to a robot catching a freely-falling object, and (iii) obstacle avoidance using a depth sensor with non-Gaussian noise. We demonstrate the ability of our approach to establish strong limits on achievable performance for these problems by comparing our upper bounds with achievable lower bounds (computed by synthesizing or learning concrete control policies).

==> sections/5multi-step.tex <==
\section{Performance Bound for Multi-Step Problems: Fano's Inequality with Feedback}
\label{sec:multi-step}

In this section, we derive an upper bound on the best achievable reward $\revision{R_{0\to T}^\star}$ defined in \eqref{eq:control problem} for the general multi time-step setting. The key idea is to extend the single-step bound from Theorem \ref{thm:single-step bound} using a dynamic programming argument. % In order to achieve this, we first extend the notion of task-relevant information (TRI) to the multi-stp case by defining the \emph{task-relevant information-to-go (TRI-TG)}. 

Let \revision{$\pi_t^k$}$: \O^{k-t+1} \rightarrow \A$ denote a policy that takes as input the sequence of observations $o_{t:k}$ from time-step $t$ to $k$ (for $k \geq t$). Thus, a policy \revision{$\pi_0^k$} at time-step $k$ utilizes all observations received up to time-step $k$. Given an initial state distribution $p_0$ and an open-loop action sequence $a_{0:t-1}$, define the reward-to-go from time $t \in \{0,\dots,T-1\}$ given  $a_{0:t-1}$ as:
\begin{equation}
\label{eq:Rt}
    \revision{R_{t\to T}} := \underset{\substack{s_{t:T-1}, o_{t:T-1} | \\ a_{0:t-1}}}{\mathbb E} \ \Bigg{[} \sum_{k=t}^{T-1} r_k(s_k, \revision{\pi_t^k}(o_{t:k})) \Bigg{]},
\end{equation}

where the expectation,
\begin{align}
    \underset{\substack{s_{t:T-1}, o_{t:T-1} | \\ a_{0:t-1}}}{\mathbb E} \  \Big{[} \cdot \Big{]} % && \underset{\substack{s_{t:T-1},\\ o_{t:T-1} | p_0,\\ a_{0:t-1}}}{\mathbb E} \  \Big{[} \cdot \Big{]}
\end{align}
is taken with respect to the distribution of states $s_{t:T-1}$ and observations $o_{t:T-1}$ one receives if one propagates $p_0$ using the open-loop sequence of actions from time-steps\endnote{For $t=0$, we use the convention that $a_{0:-1}$ is the empty sequence and:
\begin{align}
    \underset{\substack{s_{0:T-1}, o_{0:T-1} | \\ a_{0:-1}}}{\mathbb E} \  \Big{[} \cdot 
    \Big{]} \ := \underset{s_{0:T-1}, o_{0:T-1}}{\mathbb E} \  \Big{[} \cdot \Big{]}.
\end{align}} 
$0$ to $t-1$, and then applies the closed-loop policies \revision{$\pi_t^t, \pi_t^{t+1}, \dots, \pi_t^{T-1}$} from time-steps $t$ to $T-1$. 
We further define \revision{$R_{T\to T} := 0$}. 

Now, for $t \in \{0,\dots,T-1\}$, define:
\begin{equation}
\label{eq:Rt perp definition}
    \revision{R_{t\to T}^\perp} := \sup_{a_t} \ \Bigg{[} \underset{s_t|a_{0:t-1}}{\mathbb E} \Big{[} r_t(s_t, a_t) \Big{]} + R_{t+1} \Bigg{]},
\end{equation}
and 
\begin{equation}
\label{eq:Rt perp star definition}
    \revision{R_{t \to T}^{\perp \star}} := \sup_{\pi^{t+1}_{t+1}, \dots, \revision{\pi_{t+1}^{T-1}}} \revision{R_{t\to T}^\perp}.
\end{equation}

The following result then leads to a recursive structure for computing an upper bound on $\revision{R_{0\to T}^\star}$.  

\begin{restatable}[Recursive bound]{proposition}{proprecursion}
\label{prop:recursion}
For any $t = 0,\dots,T-1$, the following inequality holds for any open-loop sequence of actions $a_{0:t-1}$:
\begin{small}
\begin{equation}
\label{eq:history-dependent induction}
    \sup_{\pi^t_t, \dots, \revision{\pi_t^{T-1}}} \ \revision{R_{t\to T}} \  \leq \ \underset{\eqqcolon \tau_t(\sigma_{t:T-1}; r_{t:T-1}) }{\underbrace{(T-t) \cdot \finv \Bigg{(} \frac{\revision{R_{t\to T}^{\perp \star}}}{T-t} \ | \ \ \I_f(o_t; s_t) \Bigg{)}}}. % \nonumber
\end{equation}
\end{small}
\end{restatable}
\begin{proof}
The proof follows a similar structure to Theorem~\ref{thm:single-step bound} and is presented in Appendix \ref{app:proofs}.
\end{proof}

To see how we can use Proposition \ref{prop:recursion}, we first use \eqref{eq:control problem} and \eqref{eq:Rt} to note that the LHS of \eqref{eq:history-dependent induction} for $t=0$ is equal to $\revision{R_{0\to T}^\star}$:
 \begin{equation}
 \label{eq:R0 perp star bound}
    \revision{R_{0\to T}^\star} = \sup_{\pi^0_0, \dots, \revision{\pi_0^{T-1}}} \ \revision{ R_{0\to T}} \ \leq \ \tau_0(\sigma_{0:T-1}; r_{0:T-1}) \ .
        % R^\star = \sup_{\pi^0_0, \dots, \pi^0_{T-1}} \ \revision{ R_{0\to T}} \ \leq \ T \cdot \KLinv \Bigg{(} \frac{\revision{ R_{0\to T}}^{\perp \star}}{T} \ | \ \ \I(o_0; s_0) \Bigg{)} \ ,
\end{equation}
% where the inequality follows from \eqref{eq:history-dependent induction} for $t=0$.

The quantity $\tau_t(\sigma_{t:T-1}; r_{t:T-1})$ may be interpreted as a multi-step version of the TRIP from Definition \ref{def:TRI one-step} \revision{(which again depends on the specific choice of $f$ one uses)}. This quantity depends on the $f$-informativity $\I_f(o_t; s_t)$, which is computed using the distribution $p_t(s_t|a_{0:t-1})$ over $s_t$ that one obtains by propagating $p_0$ using the open-loop sequence of actions $a_{0:t-1}$:
%\begin{small}
\begin{equation}
\label{eq:multi-step MI}
    \I_f(o_t; s_t) = \inf_q \ \underset{\substack{s_t| \\ a_{0:t-1}}}{\mathbb E} \mathbb D_f\Big{(}\sigma_t(o_t|s_t) \| q(o_t) \Big{)}.
\end{equation}
%\end{small}

In addition, $\tau_t(\sigma_{t:T-1}; r_{t:T-1})$ depends on \revision{$ R_{t\to T}^{\perp \star}$}, which is then divided by $(T-t)$ to ensure boundedness between $[0,1]$ (see Assumption \ref{ass:bounded rewards}). The quantity \revision{$ R_{t\to T}^{\perp \star}$} can itself be upper bounded using \eqref{eq:history-dependent induction} with $t+1$, as we demonstrate below. Such an upper bound on \revision{$ R_{t\to T}^{\perp \star}$} for $t=0$ leads to an upper bound on $\revision{R_{0\to T}^\star}$ using \eqref{eq:R0 perp star bound} and the monotonicity of the $f$-inverse (Proposition~\ref{prop:f inverse properties}). Applying this argument recursively leads to Algorithm \ref{a:DP}, which computes an upper bound on $\revision{R_{0\to T}^\star}$. \revision{In Algorithm \ref{a:DP}, we use $\bar R$ to denote recursively-computed upper bounds on the RHS of \eqref{eq:history-dependent induction}.}

% \vspace{25pt}
\begin{algorithm}[H] 
% \algsetup{linenosize=\tiny}
  \caption{{\small Multi-Step Performance Bound}}
  \label{a:DP}
  \begin{algorithmic}[1]
  \STATE Initialize \revision{$\bar{R}_{T\to T}$}$(a_{0:T-1}) = 0, \ \forall a_{0:T-1}$.
  \FOR{$t = T-1, T-2, \dots, 0$}
  \STATE \revision{$ \ \forall a_{0:t-1}$, compute:} \\ \revision{$\displaystyle\bar{R}_{t\to T}(a_{0:t-1}) := (T-t) \cdot \finv\Big{(} \frac{\bar{R}_{t\to T}^{\perp \star}}{T-t} \Big{|} \I_f(o_t; s_t) \Big{)} ,$\\
  where: \\
  $\bar{R}_{t\to T}^{\perp \star} := \underset{a_t}{\sup} \ \underset{s_t|a_{0:t-1}}{\mathbb E} \Big{[} r_{t}(s_t, a_t) \Big{]} + \bar{R}_{t+1\to T}(a_{0:t}). $} \\
  % \STATE $\bar{R}_t(a_{0:t-1}) = \min\Big{\{}\bar{R}_t(a_{0:t-1}), \ T-t \Big{\}}$.
  \ENDFOR
    \RETURN \revision{$\bar{R}_{0\to T}$} (bound on achievable expected reward).
  \end{algorithmic}
\end{algorithm}





\begin{restatable}[Multi-step performance bound]{theorem}{thmmultistep}
\label{thm:multi-step bound}
Algorithm \ref{a:DP} returns an upper bound on the best achievable reward $\revision{R_{0\to T}^\star}$. 
\end{restatable}
\begin{proof}
We provide a sketch of the proof here, which uses backwards induction. In particular, Proposition \ref{prop:recursion} leads to the inductive step. See Appendix \ref{app:proofs} for the complete proof. 

We prove that for all $t=T-1,\dots,0$, 
\begin{equation}
\label{eq:algorithm bound sketch}
    \sup_{\pi^t_t, \dots, \revision{\pi_t^{T-1}}} \ \revision{R_{t\to T}} \leq \revision{\bar{R}_{t\to T}}(a_{0:t-1}), \ \forall a_{0:t-1}.
\end{equation}
Thus, in particular, 
\begin{equation}
    \revision{R_{0\to T}^\star} = \sup_{\pi^0_0, \dots, \revision{\pi_0^{T-1}}} \revision{\ R_{0\to T} \leq \bar{R}_{0\to T}}.
\end{equation}

We prove \eqref{eq:algorithm bound sketch} by backwards induction starting from $t=T-1$. We first prove the base step. Using \eqref{eq:history-dependent induction}, we obtain:
\begin{equation}
\label{eq:induction base sketch}
        \small\sup_{\pi^{T-1}_{T-1}} \ \revision{R_{T-1\to T}} \  \leq \ \finv \Big{(} \revision{R_{T-1\to T}^{\perp \star}} \ | \ \ \I_f(o_{T-1}; s_{T-1}) \Big{)}.
\end{equation}
Using the fact that \revision{$R_{T\to T} = 0$}, we can show that \revision{$R_{T-1\to T}^{\perp \star} = \bar{R}_{T-1\to T}^{\perp \star}$}. 
Combining this with \eqref{eq:induction base sketch} and the monotonicity of the $f$-inverse (Proposition \ref{prop:f inverse properties}), we see:
\begin{small}
    \begin{align}
    \sup_{\pi^{T-1}_{T-1}} \ \revision{R_{T-1\to T}} \  &\leq \ \finv \Big{(} \revision{\bar{R}_{T-1\to T}^{\perp \star}} \ | \ \ \I_f(o_{T-1}; s_{T-1}) \Big{)} \\
    &= \revision{\bar{R}_{T-1\to T}}(a_{0:T-2}).
\end{align}
\end{small}

In order to prove the induction step, suppose that for $t \in \{0,\dots,T-2\}$, we have
\begin{equation}
\label{eq:induction hypothesis sketch}
    \sup_{\pi^{t+1}_{t+1}, \dots, \revision{\pi_{t+1}^{T-1}}} \ \revision{R_{t+1\to T}} \leq \revision{\bar{R}_{t+1\to T}}(a_{0:t}).
\end{equation}
We then need to show that
\begin{equation}
\label{eq:induction WTS sketch}
    \sup_{\pi^{t}_{t}, \dots, \revision{\pi_{t}^{T-1}}} \ \revision{R_{t\to T}} \leq \revision{\bar{R}_{t\to T}}(a_{0:t-1}).
\end{equation}
We can use the induction hypothesis \eqref{eq:induction hypothesis sketch} to show that \revision{$R_{t\to T}^{\perp \star} \leq \bar{R}_{t\to T}^{\perp \star}$}. Combining this with \eqref{eq:history-dependent induction} and the monotonicity of the $f$-inverse (Proposition \ref{prop:f inverse properties}), we obtain the desired result \eqref{eq:induction WTS sketch}:
\begin{small}
\begin{align}
  \sup_{\pi^t_t, \dots, \revision{\pi_t^{T-1}}} \ \revision{R_{t\to T}} \  &\leq \ \textstyle(T-t) \cdot \finv \Bigg{(} \frac{\revision{\bar{R}_{t\to T}^{\perp \star}}}{T-t} \ | \ \ \I_f(o_t; s_t) \Bigg{)} \\
  &= \revision{\bar{R}_{t\to T}}(a_{0:t-1}).
\end{align}
\end{small}
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Full proof

% \begin{proof}
% Using (backwards) induction, we prove that for all $t=T-1,\dots,0$, 
% \begin{equation}
% \label{eq:algorithm bound}
%     \sup_{\pi^t_t, \dots, \pi^t_{T-1}} \ R_t \leq \bar{R}_t(a_{0:t-1}), \ \forall a_{0:t-1}.
% \end{equation}
% Thus, in particular, 
% \begin{equation}
%     R^\star = \sup_{\pi^0_0, \dots, \pi^0_{T-1}} \ R_0 \leq \bar{R}_0.
% \end{equation}


% We prove \eqref{eq:algorithm bound} by backwards induction starting from $t=T-1$. In particular, Proposition \ref{prop:recursion} leads to the inductive step. 

% We first prove the base step of induction using $t=T-1$. Using \eqref{eq:history-dependent induction}, we see:
% \begin{equation}
% \label{eq:induction base}
%         \sup_{\pi^{T-1}_{T-1}} \ R_{T-1} \  \leq \ \KLinv \Big{(} R_{T-1}^{\perp \star} \ | \ \ \I(o_{T-1}; s_{T-1}) \Big{)}.
% \end{equation}
% By definition (see \eqref{eq:Rt perp star definition}), 
% \begin{align}
%     R_{T-1}^{\perp \star} &= \sup_{a_{T-1}} \ \underset{s_{T-1}|p_0,a_{0:T-2}}{\mathbb E} \Big{[} r_{T-1}(s_{T-1}, a_{T-1}) \Big{]} + \underset{= 0}{\underbrace{R_{T}}} \nonumber \\
%     &= \sup_{a_{T-1}} \ \underset{s_{T-1}|p_0,a_{0:T-2}}{\mathbb E} \Big{[} r_{T-1}(s_{T-1}, a_{T-1}) \Big{]} \nonumber \\
%     &= \bar{R}_{T-1}^{\perp \star}. \nonumber
% \end{align}
% Combining this with \eqref{eq:induction base} and the monotonicity of the KL inverse (Prop. \ref{prop:kl inverse properties}), we see:
% \begin{align}
%     \sup_{\pi^{T-1}_{T-1}} \ R_{T-1} \  &\leq \ \KLinv \Big{(} \bar{R}_{T-1}^{\perp \star} \ | \ \ \I(o_{T-1}; s_{T-1}) \Big{)} \\
%     &= \bar{R}_{T-1}(a_{0:T-2}).
% \end{align}
% Next, we prove the induction step. Suppose it is the case that for $t \in \{0,\dots,T-2\}$, we have
% \begin{equation}
% \label{eq:induction hypothesis}
%     \sup_{\pi^{t+1}_{t+1}, \dots, \pi^{t+1}_{T-1}} \ R_{t+1} \leq \bar{R}_{t+1}(a_{0:t}).
% \end{equation}
% We then need to show that
% \begin{equation}
% \label{eq:induction WTS}
%     \sup_{\pi^{t}_{t}, \dots, \pi^{t}_{T-1}} \ R_{t} \leq \bar{R}_{t}(a_{0:t-1}).
% \end{equation}
% To prove this, we first observe that
% \begin{align}
%     R_t^{\perp \star} &:= \sup_{\pi_{t+1}^{t+1},\dots,\pi^{t+1}_{T-1}} \  \sup_{a_t} \ \Bigg{[} \underset{s_t|p_0,a_{0:t-1}}{\mathbb E} \Big{[} r_t(s_t, a_t) \Big{]} + R_{t+1} \Bigg{]} \nonumber \\
%     &= \sup_{a_t} \ \Bigg{[} \underset{s_t|p_0,a_{0:t-1}}{\mathbb E} \Big{[} r_t(s_t, a_t) \Big{]} + \sup_{\pi_{t+1}^{t+1},\dots,\pi^{t+1}_{T-1}} \ R_{t+1} \Bigg{]}. \nonumber
% \end{align}
% Combining this with the induction hypothesis \eqref{eq:induction hypothesis}, we see
% \begin{align}
%     R_t^{\perp \star} &\leq \sup_{a_t} \ \Bigg{[} \underset{s_t|p_0,a_{0:t-1}}{\mathbb E} \Big{[} r_t(s_t, a_t) \Big{]} + \bar{R}_{t+1}(a_{0:t}) \Bigg{]} \\
%     &\eqqcolon \bar{R}_t^{\perp \star}.
% \end{align}
% Finally, combining this with \eqref{eq:history-dependent induction} and the monotonicity of the KL inverse (Prop. \ref{prop:kl inverse properties}), we obtain the desired result \eqref{eq:induction WTS}:
% \begin{align}
%   \sup_{\pi^t_t, \dots, \pi^t_{T-1}} \ R_t \  &\leq \ (T-t) \cdot \KLinv \Bigg{(} \frac{\bar{R}_t^{\perp \star}}{T-t} \ | \ \ \I(o_t; s_t) \Bigg{)} \\
%   &= \bar{R}_{t}(a_{0:t-1}).
% \end{align}
% \end{proof}

% In order to implement Algorithm \ref{a:DP}, we can compute the KL inverse using geometric programming (see Sec. \ref{sec:kl inverse}). In addition, we require the ability to compute/bound $\I(o_t; s_t)$ and $\bar{R}_t^{\perp \star}$. We discuss these implementation aspects next. 





